An Empirical Study on Code Review Activity Prediction and Its Impact in Practice

During code reviews, an essential step in software quality assurance, reviewers have the difficult task of understanding and evaluating code changes to validate their quality and prevent introducing faults to the codebase. This is a tedious process where the effort needed is highly dependent on the code submitted, as well as the author's and the reviewer's experience, leading to median wait times for review feedback of 15-64 hours. Through an initial user study carried with 29 experts, we found that re-ordering the files changed by a patch within the review environment has potential to improve review quality, as more comments are written (+23%), and participants' file-level hot-spot precision and recall increases to 53% (+13%) and 28% (+8%), respectively, compared to the alphanumeric ordering. Hence, this paper aims to help code reviewers by predicting which files in a submitted patch need to be (1) commented, (2) revised, or (3) are hot-spots (commented or revised). To predict these tasks, we evaluate two different types of text embeddings (i.e., Bag-of-Words and Large Language Models encoding) and review process features (i.e., code size-based and history-based features). Our empirical study on three open-source and two industrial datasets shows that combining the code embedding and review process features leads to better results than the state-of-the-art approach. For all tasks, F1-scores (median of 40-62%) are significantly better than the state-of-the-art (from +1 to +9%).

==> figures/RQ1_feat.tex <==

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ1_feature_importance.png}
%          \caption{Feature importance ordered by increasing importance for each setup\Do{maybe remove this}}
%          \label{fig:RQ1_feat_val}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ1_feature_importance_cumul.png}
%          \caption{Cumulative value of the feature importance ordered by increasing importance for each setup}
%          \label{fig:RQ1_feat_cumul}
%      \end{subfigure}
     
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ1_feature_importance_WC_std_X.png}
%          \caption{Standard deviation of the actual feature values in the corpus ordered by increasing feature importance for Wordcount embeddings\Do{I could do boxes by 5-10\% of feature importance}}
%          \label{fig:RQ1_feat_WC_std}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.49\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ1_feature_importance_LLM_std_X.png}
%          \caption{Standard deviation of the actual feature values in the corpus ordered by increasing feature importance for  LLM embeddings\Do{I could do boxes by 5-10\% of feature importance}}
%          \label{fig:RQ1_feat_LLM_std}
%      \end{subfigure}
     
%         \caption{Feature analysis of best models for the different text embeddings.}
%         \label{fig:RQ1_feat}
% \end{figure}


\begin{figure}[t]
     \centering
         \includegraphics[width=.45\textwidth]{img/RQ1_feature_importance_cumul.png}
         \caption{Cumulative value of the feature importance ordered by increasing importance for each setup}
         \label{fig:RQ1_feat_cumul}
     
\end{figure}

==> figures/RQ1and2.tex <==
\begin{figure}[h]
     \centering

     \begin{minipage}[c]{.7\textwidth}
         \includegraphics[width=\textwidth]{img/RQ1_feature_importance_cumul.png}
         \caption{Cumulative tendencies value of the feature importance ordered by increasing importance for each setup.}
         \label{fig:RQ1_feat_cumul}
     \end{minipage}
     % \hfill
 \end{figure}
 \begin{figure}[h]
      \centering
     \begin{minipage}[c]{.7\textwidth}
     \centering
     \includegraphics[width=\textwidth]{img/RQ2_feature_importance.png}
         \caption{Feature importance [\%] by type of features with the 'All' approach.}
         \label{fig:RQ2_all_imp}
     \end{minipage}
\end{figure}

==> figures/RQ2_feat.tex <==
% \begin{figure}[t]
%      \centering
%      \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ2_feature_importance.png}
%          \caption{Feature importance [\%] by type of features with the 'All' approach.}
%          \label{fig:RQ2_all_imp}
%      \end{subfigure}
%      \hfill
%      % \begin{subfigure}[b]{0.49\textwidth}
%      %     \centering
%      %     \includegraphics[width=\textwidth]{img/RQ2_number_feature_importance_75.png}
%      %     \caption{Number of features if we only kept top 25\% of features.}
%      %     \label{fig:RQ2_all_imp_count_75}
%      % \end{subfigure}
%      % % \hfill
%      % % \begin{subfigure}[b]{0.49\textwidth}
%      % %     \centering
%      % %     \includegraphics[width=\textwidth]{img/RQ2_perc_feature_importance_75.png}
%      % %     \caption{Feature importance [\%] if we only kept top 25\% of features.}
%      % %     \label{fig:RQ2_all_imp_perc_75}
%      % % \end{subfigure}
%       \begin{subfigure}[b]{0.45\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{img/RQ2_experience.png}
%          \caption{Maximum experience by target and by dataset.\\}
%          \label{fig:RQ2_experience}
%      \end{subfigure}
    
%         \caption{Feature analysis of best models for the different review process feature embeddings.}
%         \label{fig:RQ2_feat}
% \end{figure}

\begin{figure}[t]
     \centering
     \includegraphics[width=.5\textwidth]{img/RQ2_feature_importance.png}
         \caption{Feature importance [\%] by type of features with the 'All' approach.}
         \label{fig:RQ2_all_imp}
\end{figure}

==> figures/ex_patch.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.7\textwidth]{img/patch_small.pdf}
    \caption{Patch example from the Base dataset. The patch number is 307497 and has three changed files. The second changed file is open as to show the actual changes: the user-interface shows the code's old version on the left and the new version on the right, where the green text is the added code and the red text is removed. In this example, the initial commit of the patch is shown (commit number 98b61b0).~\cite{expatch}}
    \label{fig:patch}
\end{figure}

==> tables/RQ1_res.tex <==

% % \begin{landscape}
% \begin{table}[h]
% % \begin{sidewaystable}
%     \centering

%     \caption{Results of text embeddings on the code review activity prediction task. The results are returned for the best model ("mod") for each setting of text embedding. Darker blue cells indicate the maximum values for each metric by dataset and the light blue cells indicate values not significantly different from the maximum value. \Do{need to fix the statistical test for Closed1 and 2}}
%     \label{RQ1:res}
%     \begin{tabular}{ll|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c}
%         &\multicolumn{1}{c|}{Text}
%         &\multicolumn{6}{c|}{commented}& \multicolumn{6}{c}{revised}& \multicolumn{6}{c}{revised}
%         \\
%         & \multicolumn{1}{c|}{Embed}
%         &auc&f1&gm&pre&rec&mod
%         &auc&f1&gm&pre&rec&mod
%         &auc&f1&gm&pre&rec&mod
%         \\


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
% &WC +
% &64& 38& 60& 30\bestcell & 50&RFs&68& 42& 63& 34\samecell & 55\samecell &RFs&65& 48\samecell & 62\samecell & 41\samecell & 59\samecell &RFs\\ 
% &WC +/-
% &64& 38& 61& 30\samecell & 52&RFs&69\bestcell & 43\samecell & 64\bestcell & 32& 66\bestcell &RFs&65& 49\samecell & 62\samecell & 40\samecell & 62\bestcell &RFs\\ 
% &LLM +
% &67\bestcell & 39\bestcell & 63\bestcell & 28& 66\bestcell &RFs&68\samecell & 43\bestcell & 63& 36\bestcell & 53&RFs&66\bestcell & 49\bestcell & 62\bestcell & 42\bestcell & 58\samecell &RFs\\ 
% &LLM +/-
% &66\samecell & 39\samecell & 63\samecell & 28& 66\samecell &RFs&68\samecell & 42\samecell & 64& 31\samecell & 64\samecell &RFs&66\samecell & 49\samecell & 62\samecell & 42\samecell & 59\samecell &RFs\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
% &WC +
% &78& 46& 69& 37\samecell & 60\samecell &RFs&68& 49\bestcell & 65\samecell & 35& 78\bestcell &RFs&71& 56\bestcell & 66\samecell & 43& 78\samecell &RFs\\ 
% &WC +/-
% &78& 46\samecell & 70\samecell & 38\bestcell & 60\samecell &RFs&69\bestcell & 48\samecell & 66\bestcell & 37\bestcell & 69&RFs&71& 55& 64& 41& 83\bestcell &RF\\ 
% &LLM +
% &79\bestcell & 48\bestcell & 72\samecell & 36\samecell & 69\bestcell &RFs&67& 46& 63& 33& 74&RFs&72\samecell & 55\samecell & 67\bestcell & 45\bestcell & 71&RF\\ 
% &LLM +/-
% &78& 47\samecell & 72\bestcell & 35\samecell & 67\samecell &RFs&67& 46& 63& 33& 75&RFs&72\bestcell & 55& 66\samecell & 43\samecell & 74&RFs\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
% &WC +
% &77& 64& 74& 56\samecell & 74\bestcell &RFs&76& 47& 66\samecell & 42\samecell & 52\samecell &RFs&62\samecell & 61\samecell & 48\samecell & 45\samecell & 93&RFs\\ 
% &WC +/-
% &78\bestcell & 65\bestcell & 75\bestcell & 59\samecell & 73\samecell &RFs&77& 47& 68\bestcell & 40\samecell & 59\bestcell &RFs&64\bestcell & 61\bestcell & 51\bestcell & 46\bestcell & 92&RFs\\ 
% &LLM +
% &77& 63& 73& 60\bestcell & 68\samecell &RFs&77\samecell & 47& 66\samecell & 44\samecell & 51\samecell &RFs&58& 59& 30& 42& 98\bestcell &RF\\ 
% &LLM +/-
% &77\samecell & 63& 74& 60\samecell & 67\samecell &RFs&78\bestcell & 48\bestcell & 66\samecell & 44\bestcell & 52\samecell &RFs&58& 59& 33& 43& 98&RFs\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
% &WC +
% &74\samecell & 37\bestcell & 64\samecell & 30\samecell & 47\samecell &RFs&71\samecell & 44\samecell & 65\samecell & 38\samecell & 58\samecell &RFs&67\samecell & 51\samecell & 63\samecell & 43\samecell & 72\samecell &RF\\ 
% &WC +/-
% &74\samecell & 37\samecell & 65\samecell & 31\bestcell & 49\samecell &RFs&72\bestcell & 45\bestcell & 66\bestcell & 38\bestcell & 57\samecell &RFs&67\samecell & 51\samecell & 62\samecell & 41\samecell & 68&RFs\\ 
% &LLM +
% &76\bestcell & 36\samecell & 66\bestcell & 30\samecell & 51\samecell &RFs&71\samecell & 45\samecell & 65\samecell & 36\samecell & 62\samecell &RFs&69\samecell & 54\bestcell & 63\samecell & 44\bestcell & 75\bestcell &RFs\\ 
% &LLM +/-
% &74\samecell & 36\samecell & 66\samecell & 26\samecell & 55\bestcell &RFs&71\samecell & 45\samecell & 66\samecell & 34\samecell & 67\bestcell &RFs&69\bestcell & 53\samecell & 63\bestcell & 43\samecell & 68\samecell &RFs\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
% &WC +
% &71& 33\samecell & 60\samecell & 27\bestcell & 42&RFs&68\samecell & 40\samecell & 64& 33\samecell & 52&RFs&67\samecell & 49\samecell & 62\samecell & 39\samecell & 68\samecell &RFs\\ 
% &WC +/-
% &74\samecell & 34\bestcell & 63\samecell & 27\samecell & 45\samecell &RFs&70\samecell & 41\samecell & 65\samecell & 33\samecell & 58&RFs&67\samecell & 50\samecell & 63\samecell & 39\samecell & 71\samecell &RFs\\ 
% &LLM +
% &75\samecell & 33\samecell & 63\samecell & 26\samecell & 50\bestcell &RFs&71\samecell & 43\bestcell & 65\samecell & 34\samecell & 62\samecell &RFs&68\samecell & 52\bestcell & 62\samecell & 42\bestcell & 74\bestcell &RFs\\ 
% &LLM +/-
% &77\bestcell & 34\samecell & 64\bestcell & 26\samecell & 48\samecell &RFs&73\bestcell & 42\samecell & 67\bestcell & 34\bestcell & 65\bestcell &RFs&71\bestcell & 52\samecell & 63\bestcell & 41\samecell & 72\samecell &RFs\\ 

%     \end{tabular}
% % \end{sidewaystable}
% \end{table}


% \begin{landscape}
\begin{table}[t]
% \begin{sidewaystable}
    \centering
\small
    \caption{Results of text embeddings on the code review activity prediction task. The results are returned for the best model ("mod") for each setting of text embedding. The results of the median F1-score are reported. Blue cells indicate the maximum values for each metric by dataset and by label.}
    \label{RQ1:res}
    % \begin{tabular}{ll
    % |p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c
    % |p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c
    % |p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c}
    \begin{tabularx}{\textwidth}{Xl|XXXXXc|XXXXXc|XXXXXc}
       \hline
        &\multicolumn{1}{c|}{\textbf{Text}}
        &\multicolumn{6}{c|}{\textbf{Commented}}& \multicolumn{6}{c|}{\textbf{Revised}}& \multicolumn{6}{c}{\textbf{Hot-spot}}
        \\
        & \multicolumn{1}{c|}{\textbf{Embed}}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        \\


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
% &WC +
% &64& 38& 60& 30\bestcell & 50&RFs&68& 42& 63& 34\samecell & 55\samecell &RFs&65& 48\samecell & 62\samecell & 41\samecell & 59\samecell &RFs\\ 
% &WC +/-
% &64& 38& 61& 30\samecell & 52&RFs&69\bestcell & 43\samecell & 64\bestcell & 32& 66\bestcell &RFs&65& 49\samecell & 62\samecell & 40\samecell & 62\bestcell &RFs\\ 
% &LLM +
% &67\bestcell & 39\bestcell & 63\bestcell & 28& 66\bestcell &RFs&68\samecell & 43\bestcell & 63& 36\bestcell & 53&RFs&66\bestcell & 49\bestcell & 62\bestcell & 42\bestcell & 58\samecell &RFs\\ 
% &LLM +/-
% &66\samecell & 39\samecell & 63\samecell & 28& 66\samecell &RFs&68\samecell & 42\samecell & 64& 31\samecell & 64\samecell &RFs&66\samecell & 49\samecell & 62\samecell & 42\samecell & 59\samecell &RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
&BoW~+
&64& 11& 24& 42\bestcell & 6&RFs&68& 36& 53& 43& 31&RFs&65& 45& 59& 47\bestcell & 44&RFs\\ 
\cline{2-20}   
&BoW~+/-
&62& 10& 23& 33& 6&RF&69\bestcell & 31& 46& 44\bestcell & 23&RFs&66\bestcell & 46& 60& 46& 47&RFs\\ 
&LLM~+
&67\bestcell & 33& 51\bestcell & 39& 29&RFs&68& 41\bestcell & 59\bestcell & 41& 42\bestcell &RFs&66\bestcell & 47& 61& 47\bestcell & 47&RFs\\ 
&LLM~+/-
&66& 34\bestcell & 51\bestcell & 39& 30\bestcell &RFs&68& 41\bestcell & 59\bestcell & 39& 42\bestcell &RFs&66\bestcell & 48\bestcell & 62\bestcell & 42& 57\bestcell &RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
&BoW~+
&78& 46& 69& 38& 58\bestcell &RFs&67& 42& 61& 36& 52&RFs&71& 54\bestcell & 66& 44& 69&RFs\\ 
\cline{2-20}   
&BoW~+/-
&79\bestcell & 45& 68& 36& 57&RFs&69\bestcell & 46\bestcell & 64\bestcell & 39& 56\bestcell &RFs&71& 54\bestcell & 66& 44& 70&RFs\\ 
&LLM~+
&79\bestcell & 48\bestcell & 70\bestcell & 42\bestcell & 57&RFs&67& 22& 37& 45\bestcell & 15&RFs&71& 54\bestcell & 66& 44& 74\bestcell &RFs\\ 
&LLM~+/-
&78& 45& 67& 40& 53&RFs&67& 23& 38& 43& 15&RFs&72\bestcell & 54\bestcell & 67\bestcell & 47\bestcell & 63&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
&BoW~+
&76& 33& 47& 52& 24&RFs&76& 46& 65& 42& 51&RFs&62& 47& 56& 51& 44&RFs\\ 
\cline{2-20}   
&BoW~+/-
&78\bestcell & 35\bestcell & 48\bestcell & 57& 25\bestcell &RFs&77& 47& 66& 43& 52&RFs&63\bestcell & 48& 57\bestcell & 53\bestcell & 44&RFs\\ 
&LLM +
&77& 32& 45& 59& 22&RFs&78\bestcell & 47& 68\bestcell & 38& 61\bestcell &RFs&58& 48& 56& 47& 52\bestcell &RFs\\ 
&LLM +/-
&77& 32& 46& 60\bestcell & 22&RFs&78\bestcell & 48\bestcell & 66& 44\bestcell & 52&RFs&58& 50\bestcell & 57\bestcell & 48& 51&RF\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
&BoW +
&74& 26& 42& 40& 18&RFs&71& 26& 42& 50& 19&RFs&67& 47\bestcell & 59& 51& 40&RFs\\ 
\cline{2-20}  
&BoW +/-
&74& 25& 42& 41\bestcell & 18&RFs&72\bestcell & 25& 39& 54\bestcell & 16&RFs&67& 43& 57& 56\bestcell & 39&RFs\\ 
&LLM +
&76\bestcell & 31\bestcell & 54\bestcell & 33& 33\bestcell &RFs&71& 36\bestcell & 51\bestcell & 46& 28\bestcell &RFs&69\bestcell & 46& 61\bestcell & 53& 45\bestcell &RFs\\ 
&LLM +/-
&74& 30& 53& 31& 31&RFs&71& 31& 47& 44& 23&RFs&69\bestcell & 46& 60& 53& 43&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
&BoW +
&71& 21& 37& 34\bestcell & 14&RFs&68& 30& 47& 42& 23&RFs&67& 46& 60& 47& 45&RFs\\ 
\cline{2-20} 
&BoW +/-
&74& 22& 40& 33& 17&RFs&70& 28& 44& 43& 21&RFs&67& 46& 60& 45& 47&RFs\\ 
&LLM +
&75& 23& 44& 30& 22&RFs&71& 35& 53\bestcell & 44& 31\bestcell &RFs&68& 45& 60& 48& 54\bestcell &RFs\\ 
&LLM +/-
&77\bestcell & 26\bestcell & 52\bestcell & 31& 30\bestcell &RFs&73\bestcell & 37\bestcell & 53\bestcell & 48\bestcell & 29&RFs&71\bestcell & 49\bestcell & 64\bestcell & 49\bestcell & 52&RFs\\ 

\hline 

    \end{tabularx}
    % \end{tabular}
% \end{sidewaystable}
\end{table}


==> tables/RQ1_stats.tex <==
\begin{table}[t]
% \begin{sidewaystable}
    \centering
    \small
    \caption{Stat RQ1.\Do{will be flipped to label X (Comparison X metric)}}
    \label{RQ1:res}
    \begin{tabular}{ll|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}}
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{4}{c|}{commented}& \multicolumn{4}{c|}{revised}& \multicolumn{4}{c}{hot-spot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        \\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{all}}}

& BoW + vs BoW +/-
&$+$ smal & .003& & .604&$+$ smal & .000& & .441& & .059& & .064\\
& BoW + vs LLM +
&$+$ smal & .009& & .076&$+$ smal & .004& & .499& & .637& & .177\\
& BoW +/- vs LLM +/-
& & .224& & .040& & .722& & .454& & .550& & .012\\
& BoW +/- vs best text
& & .021& & .027& & .139&$+$ smal & .001& & .399&$+$ smal & .003\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& BoW + vs BoW +/-
& & .934& & .762&$+$ larg & .000& & .151& & .041&$+$ smal & .003\\
& BoW + vs LLM +
&$+$ medi & .000& & .055& & .048& & .561& & .561& & .073\\
& BoW +/- vs LLM +/-
& & .421& & .359& & .454& & .720& & .804& & .012\\
& BoW +/- vs best text
&$+$ smal & .005& & .017& & .114& & .017& & .203&$+$ smal & .007\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& BoW + vs BoW +/-
&$+$ smal & .001& & .633&$+$ smal & .000& & .759& & .412& & .609\\
& BoW + vs LLM +
& & .320& & .812& & .089& & .147& & .272& & .759\\
& BoW +/- vs LLM +/-
& & .579& & .329& & .818& & .120& & .120& & .225\\
& BoW +/- vs best text
& & .495& & .468& & .347& & .018& & .702& & .038\\
    


% WITH VALIDATION
\\\\ \hline \hline
& BoW + vs BoW +/-
&$+$ smal & .000& & .024&$+$ smal & .000& & .441& & .396& & .078\\
& BoW + vs LLM +
& & .028& & .405& & .053& & .016& & .388& & .012\\
& BoW +/- vs LLM +/-
& & .322& & .054& & .304& & .038&$+$ smal & .000&$+$ smal & .001\\
& BoW +/- vs best text
& & .121& & .615& & .136&$+$ smal & .007& & .106&$+$ smal & .007\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& BoW + vs BoW +/-
&$+$ smal & .001& & .074& & .012& & .804& & .095& & .359\\
& BoW + vs LLM +
&$+$ medi & .000& & .847& & .330& & .169&$+$ smal & .004&$+$ medi & .004\\
& BoW +/- vs LLM +/-
& & .135&$-$ smal & .004& & .720& & .169&$+$ smal & .002& & .095\\
& BoW +/- vs best text
& & .080& & .000&$+$ smal & .008& & .012& & .012& & .010\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& BoW + vs BoW +/-
&$+$ smal & .001& & .137&$+$ smal & .000& & .609& & .892& & .157\\
& BoW + vs LLM +
& & .609& & .229& & .128& & .065& & .452& & .191\\
& BoW +/- vs LLM +/-
& & .000& & .854& & .404& & .120& & .035&$+$ medi & .002\\
& BoW +/- vs best text
& & .369& & .495& & .000& & .111& & .932& & .119\\


\end{tabular}
% \end{sidewaystable}
\end{table}

==> tables/RQ2_mega_res.tex <==


\begin{table}[t]
    \centering

    \caption{Results of software meta-features embeddings on the code review activity prediction task. The results are returned for the best model ("mod") for each setting of text embedding. Darker blue cells indicate the maximum values for each metric by dataset and the light blue cells indicate values not significantly different from the maximum value.}
    \label{tab:RQ2_res}
    
    \begin{tabular}{ll|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c}
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{6}{c|}{commented}& \multicolumn{6}{c}{revised}& \multicolumn{6}{c}{Hotspot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        \\



\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
& Best text
&67\bestcell & 29& 45& 41& 22&RFs&69& 37\bestcell & 54\bestcell & 46& 33\bestcell &RFs&67& 44\bestcell & 57\bestcell & 53& 37\bestcell &RFs\\ \cline{2-20}
&\#Add/Rem
&57& 14& 29& 39& 9&RF&65& 24& 40& 40& 17&RF&62& 27& 41& 46& 19&RF\\ 
&Count
&62& 32\bestcell & 52\bestcell & 31& 34\bestcell &RFs&65& 28& 44& 40& 21&RF&65& 34& 49& 46& 27&RF\\ 
&Hist
&57& 19& 37& 25& 15&RFs&63& 12& 26& 40& 7&RF&60& 37& 52& 41& 35&RFs\\ 
&All
&67& 8& 21& 58\bestcell & 5&RF&74\bestcell & 28& 42& 61\bestcell & 18&RF&70\bestcell & 37& 49& 61\bestcell & 26&RF\\ 


\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
& Best text
&80\bestcell & 44\bestcell & 63\bestcell & 45\bestcell & 44\bestcell &RFs&70& 44\samecell & 61& 42& 46&RFs&72& 55\bestcell & 67\bestcell & 48& 64\samecell &RFs\\ \cline{2-20}
&\#Add/Rem
&57& 20& 39& 23& 17&RF&60& 34& 52& 34& 33&RF&63& 45& 59& 43& 47&RF\\ 
&Count
&69& 23& 39& 37& 16&RF&66& 44\bestcell & 62\bestcell & 36& 57\bestcell &RFs&66& 49& 61& 40& 65\bestcell &RFs\\ 
&Hist
&65& 7& 19& 44& 4&RF&66& 15& 30& 40& 10&RF&67& 31& 45& 55\samecell & 22&RF\\ 
&All
&76& 4& 15& 40& 2&RF&74\bestcell & 38& 53& 50\bestcell & 31&RFs&77\bestcell & 52& 64& 57\bestcell & 48&RFs\\ 


\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
& Best text
&78\bestcell & 29\bestcell & 43\samecell & 62& 19&RFs&78\bestcell & 47\bestcell & 63\samecell & 51\bestcell & 44&RFs&64\bestcell & 45\bestcell & 55\bestcell & 62\bestcell & 36&RFs\\ \cline{2-20}
&\#Add/Rem
&58& 29\samecell & 44\bestcell & 40& 23\bestcell &RFs&71& 30& 47& 37& 25&RF&57& 43& 53& 52& 37\bestcell &RFs\\ 
&Count
&48& 19& 33& 52& 12&RF&75& 39& 58& 38& 40&RFs&52& 41& 52& 55& 32&RF\\ 
&Hist
&57& 6& 18& 48& 3&RF&70& 40& 61& 36& 47\bestcell &RFs&58& 37& 48& 45& 32&RF\\ 
&All
&53& 16& 30& 66\bestcell & 9&RF&78\samecell & 46\samecell & 63\bestcell & 46& 46\samecell &RFs&55& 42& 53& 60\samecell & 32&RF\\ 


\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
& Best text
&83\bestcell & 28\bestcell & 44\bestcell & 100\bestcell & 20\bestcell &RFs&80& 33\bestcell & 48\bestcell & 75\bestcell & 25\bestcell &RFs&80\samecell & 43\bestcell & 52\bestcell & 100\bestcell & 31\bestcell &RF\\ \cline{2-20}
&\#Add/Rem
&&&&&&&&&&&&&&&&&&\\ 
&Count
&&&&&&&&&&&&&&&&&&\\ 
&Hist
&79& 1& 7& 50& 0&RF&81\bestcell & 32& 45& 60& 22&RF&84\bestcell & 30& 45& 62& 22&RF\\ 
&All
&&&&&&&&&&&&&&&&&&\\ 


\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
& Best text
&81\bestcell & 25& 42& 42\bestcell & 18&RFs&85\bestcell & 67\bestcell & 75\bestcell & 80\bestcell & 57&RFs&79\bestcell & 61\bestcell & 69\bestcell & 68\bestcell & 59&RFs\\ \cline{2-20}
&\#Add/Rem
&&&&&&&&&&&&&&&&&&\\ 
&Count
&&&&&&&&&&&&&&&&&&\\ 
&Hist
&67& 27\bestcell & 63\bestcell & 18& 71\bestcell &RFs&69& 39\samecell & 66\samecell & 26& 83\bestcell &RFs&71& 56\samecell & 63& 42& 90\bestcell &RFs\\ 
&All
&&&&&&&&&&&&&&&&&&\\ 




    \end{tabular}
    
\end{table}


==> tables/RQ2_res.tex <==


\begin{table}[t]
    \centering
    \small
    \caption{Results of software review process features embeddings on the code review activity prediction tasks. The results are returned for the best model ("mod") for each setting of text embedding. The results of the median F1-score are reported. Blue cells indicate the maximum values for each metric by dataset and by label.}
    \label{tab:RQ2_res}
    
    \begin{tabularx}{\textwidth}{Xl|XXXXXc|XXXXXc|XXXXXc}
    \hline
        &\multicolumn{1}{c|}{\textbf{Text}}
        &\multicolumn{6}{c|}{\textbf{Commented}}& \multicolumn{6}{c|}{\textbf{Revised}}& \multicolumn{6}{c}{\textbf{Hot-spot}}
        \\
        & \multicolumn{1}{c|}{\textbf{Embed}}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        \\

% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
% & Best text
% &67\bestcell & 39\bestcell & 63\bestcell & 28\samecell & 66\samecell &RFs&69& 43& 64& 32\samecell & 66\samecell &RFs&66& 49& 62\samecell & 42\bestcell & 58&RFs\\ \cline{2-20}
% &Add/Rem
% &57& 33& 56& 25& 47&RF&65& 40& 62& 29& 64\samecell &RF&62& 48& 56& 35& 76&RF\\ 
% &Count
% &62& 36& 59& 26& 60&RFs&65& 40& 62& 29& 66\samecell &RF&64& 48& 55& 35& 79&RF\\ 
% &Hist
% &57& 33& 51& 21& 76\bestcell &RFs&63& 38& 57& 26& 73\bestcell &RF&60& 46& 28& 30& 97\bestcell &RFs\\ 
% &All
% &66\samecell & 38\samecell & 61& 29\bestcell & 56&RF&73\bestcell & 45\bestcell & 66\bestcell & 36\bestcell & 62\samecell &RF&70\bestcell & 51\bestcell & 63\bestcell & 40\samecell & 73&RF\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
% & Best text
% &79\bestcell & 48\bestcell & 72\bestcell & 36\bestcell & 69&RFs&69& 48& 66& 37\samecell & 69\samecell &RFs&72& 55& 66\samecell & 43\bestcell & 74&RFs\\ \cline{2-20}
% &Add/Rem
% &57& 30& 56& 19& 69&RF&60& 41& 56& 28& 72\samecell &RF&63& 48& 56& 35& 75&RF\\ 
% &Count
% &69& 38& 66& 27& 66\samecell &RF&65& 43& 60& 38\bestcell & 53&RFs&66& 50& 60& 38& 73&RFs\\ 
% &Hist
% &64& 33& 60& 22& 71\bestcell &RF&65& 43& 60& 31& 67\samecell &RF&66& 50& 51& 35& 86\bestcell &RF\\ 
% &All
% &75& 41& 66& 32& 54&RF&73\bestcell & 49\bestcell & 67\bestcell & 37\samecell & 73\bestcell &RFs&76\bestcell & 57\bestcell & 67\bestcell & 43\samecell & 84\samecell &RFs\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
% & Best text
% &78\bestcell & 65\bestcell & 75\bestcell & 59\bestcell & 73&RFs&78\bestcell & 48\bestcell & 66\samecell & 44\bestcell & 52&RFs&64\bestcell & 61\bestcell & 51\bestcell & 46\bestcell & 92&RFs\\ \cline{2-20}
% &Add/Rem
% &56& 50& 55& 36& 82&RFs&70& 43& 66& 34& 58&RF&57& 59& 40& 43& 94\bestcell &RFs\\ 
% &Count
% &47& 39& 53& 36& 43&RF&75& 45& 69\samecell & 34& 73\bestcell &RFs&52& 48& 49\samecell & 40& 59&RF\\ 
% &Hist
% &55& 47& 44& 33& 88\bestcell &RF&66& 41& 63& 33& 54&RFs&57& 58& 45& 44& 89\samecell &RF\\ 
% &All
% &51& 41& 55& 39& 41&RF&77\samecell & 48\samecell & 70\bestcell & 37\samecell & 66\samecell &RFs&54& 53& 19& 38& 85\samecell &RF\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
% & Best text
% &76\bestcell & 36\bestcell & 66\bestcell & 30\bestcell & 51&RFs&72\bestcell & 45\bestcell & 66\bestcell & 38\bestcell & 57&RFs&69\bestcell & 53\bestcell & 63\bestcell & 43\bestcell & 68&RFs\\ \cline{2-20}
% &Add/Rem
% &&&&&&&&&&&&&&&&&&\\ 
% &Count
% &&&&&&&&&&&&&&&&&&\\ 
% &Hist
% &59& 27& 54\samecell & 15& 78\bestcell &RF&59& 37& 41& 23& 96\bestcell &RF&61\samecell & 51\samecell & 34& 35& 99\bestcell &RF\\ 
% &All
% &&&&&&&&&&&&&&&&&&\\ 


% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
% & Best text
% &77\bestcell & 34\bestcell & 64\bestcell & 26\bestcell & 48\samecell &RFs&73\bestcell & 42\bestcell & 67\bestcell & 34\bestcell & 65&RFs&71\bestcell & 52\bestcell & 63\bestcell & 41\bestcell & 72\samecell &RFs\\ \cline{2-20}
% &Add/Rem
% &&&&&&&&&&&&&&&&&&\\ 
% &Count
% &&&&&&&&&&&&&&&&&&\\ 
% &Hist
% &60& 22& 57\samecell & 13& 71\bestcell &RFs&62& 36& 59& 24\samecell & 74\bestcell &RFs&66\samecell & 50\samecell & 63\samecell & 38\samecell & 77\bestcell &RFs\\ 
% &All
% &&&&&&&&&&&&&&&&&&\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
& Best text
&66\bestcell & 34\bestcell & 51& 39\bestcell & 30&RFs&68& 41& 59& 41\bestcell & 42&RFs&66& 48& 62& 42& 57&RFs\\ \cline{2-20}
&Add/Rem
&54& 25& 44& 29& 22&RFs&60& 35& 55& 32& 38&RFs&59& 41& 56& 40& 43&RFs\\ 
&Count
&62& 33& 54\bestcell & 29& 38\bestcell &RFs&64& 38& 59& 32& 48&RFs&64& 45& 59& 40& 51&RFs\\ 
&Hist
&59& 29& 51& 24& 36&RFs&63& 37& 59& 30& 55\bestcell &RFs&59& 43& 55& 35& 62\bestcell &RFs\\ 
&All feat
&66\bestcell & 33& 51& 37& 30&RFs&72\bestcell & 45\bestcell & 64\bestcell & 41\bestcell & 52&RFs&69\bestcell & 51\bestcell & 64\bestcell & 46\bestcell & 57&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
& Best text
&79\bestcell & 48\bestcell & 70\bestcell & 42& 57\bestcell &RFs&69& 46\bestcell & 64\bestcell & 39& 56&RFs&71& 54\bestcell & 66\bestcell & 44& 70\bestcell &RFs\\ \cline{2-20}
&Add/Rem
&56& 27& 53& 20& 42&RFs&60& 39& 58& 31& 51&RF&63& 46& 58& 36& 64&RF\\ 
&Count
&67& 30& 56& 24& 41&RFs&65& 41& 60& 33& 60\bestcell &RFs&66& 47& 60& 41& 57&RF\\ 
&Hist
&63& 27& 53& 23& 37&RFs&74& 24& 40& 49& 17&RF&71& 47& 60& 50& 45&RFs\\ 
&All feat
&72& 14& 28& 45\bestcell & 8&RFs&75\bestcell & 19& 33& 68\bestcell & 11&RFs&76\bestcell & 26& 40& 67\bestcell & 16&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
& Best text
&78\bestcell & 35& 48& 57& 25&RFs&78\bestcell & 48\bestcell & 66\bestcell & 44& 52&RFs&58& 50& 57& 48& 51&RF\\ \cline{2-20}
&Add/Rem
&56& 30& 46& 36& 26&RFs&69& 43& 65& 35& 56\bestcell &RFs&57& 47& 55& 47& 46&RF\\ 
&Count
&46& 32& 47& 42& 26&RFs&75& 40& 61& 36& 45&RFs&52& 44& 53& 49& 39&RFs\\ 
&Hist
&72& 54\bestcell & 65\bestcell & 47& 67\bestcell &RF&66& 37& 57& 34& 40&RFs&64\bestcell & 55\bestcell & 61\bestcell & 52& 58\bestcell &RFs\\ 
&All feat
&54& 20& 34& 59\bestcell & 12&RFs&77& 37& 52& 50\bestcell & 29&RFs&55& 41& 52& 57\bestcell & 32&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
& Best text
&76\bestcell & 31& 54& 33\bestcell & 33&RFs&71& 36& 51& 46\bestcell & 28&RFs&67& 47& 59& 51\bestcell & 40&RFs\\ \cline{2-20}
&Add/Rem
&60& 21& 47& 20& 25&RFs&67& 36& 57& 34& 39&RF&59& 45& 55& 36& 66\bestcell &RFs\\ 
&Count
&75& 32& 56& 32& 35&RFs&76& 42& 62& 42& 45&RFs&69& 49& 60& 48& 50&RFs\\ 
&Hist
&56& 24& 53& 16& 46\bestcell &NBs&60& 33& 55& 26& 46&NBs&59& 41& 55& 38& 47&NBs\\ 
&All feat
&76\bestcell & 33\bestcell & 57\bestcell & 30& 34&RFs&77\bestcell & 44\bestcell & 64\bestcell & 44& 48\bestcell &RFs&71\bestcell & 55\bestcell & 65\bestcell & 50& 59&RFs\\ 


\hline 
\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
& Best text
&77& 26& 52& 31& 30&RFs&73& 37& 53& 48\bestcell & 29&RFs&71& 49& 64& 49\bestcell & 52&RFs\\ \cline{2-20}
&Add/Rem
&69& 21& 42& 24& 19&RF&67& 36& 57& 31& 38&RF&62& 44& 59& 36& 58\bestcell &RF\\ 
&Count
&78& 29& 52& 33\bestcell & 29&RFs&74& 39& 59& 40& 41&RFs&70& 46& 60& 45& 48&RFs\\ 
&Hist
&61& 20& 56& 13& 48\bestcell &NBs&63& 34& 58& 25& 50\bestcell &NBs&64& 44& 59& 39& 51&NBs\\ 
&All feat
&79\bestcell & 34\bestcell & 58\bestcell & 29& 37&RFs&77\bestcell & 42\bestcell & 62\bestcell & 42& 45&RFs&74\bestcell & 52\bestcell & 65\bestcell & 47& 57&RFs\\ 

\hline 



    \end{tabularx}
    
\end{table}


==> tables/RQ2_res_selection.tex <==

\begin{table}[h!]
    \centering
    \caption{Results of software meta-features embeddings with feature selection on the code review activity prediction task. The results are returned for the best model ("mod") for each setting of text embedding. Darker blue cells indicate the maximum values for each metric by dataset and the light blue cells indicate values not significantly different from the maximum value.}
    \label{tab:RQ2_res_selection}
    
    \begin{tabular}{ll|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c}
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{6}{c|}{commented}& \multicolumn{6}{c}{revised}& \multicolumn{6}{c}{Hotspot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        \\
\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Base }}}

& All
&67\bestcell & 8& 21& 58\bestcell & 5& RF&74\bestcell & 28\bestcell & 42& 61\bestcell & 18& RF&70\bestcell & 37\samecell & 49& 61\bestcell & 26& RF\\

\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Ironic }}}
& All
&76\bestcell & 4& 15& 40\bestcell & 2& RF&74\bestcell & 38& 53& 50\bestcell & 31& RFs&77\bestcell & 52& 64& 57\bestcell & 48& RFs\\

\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Nova }}}
& All
&53& 16& 30& 66\bestcell & 9& RF&78\bestcell & 46\bestcell & 63\bestcell & 46\bestcell & 46\samecell & RFs&55& 42& 53& 60\bestcell & 32& RF\\

\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Closed1 }}}
& All
&&&&&&&&&&&&&&&&&&\\

\hline
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{ Closed2 }}}
& All
&&&&&&&&&&&&&&&&&&\\


    \end{tabular}

\end{table}

==> tables/RQ2_stats.tex <==
\begin{table}[t]
% \begin{sidewaystable}
    \centering
\small
    \caption{Stat RQ2.}
    \label{RQ1:res}
        \begin{tabular}{ll|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}}
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{4}{c|}{commented}& \multicolumn{4}{c}{revised}& \multicolumn{4}{c}{hot-spot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        \\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{all}}}

& best text vs \#Add/Rem
&$-$ larg & .000&$-$ larg & .004&$-$ larg & .000& & .016&$-$ larg & .000&$-$ larg & .001\\
& best text vs Count
& & .031& & .492& & .728& & .893& & .067& & .048\\
& best text vs Hist
&$-$ larg & .000& & .045&$-$ larg & .000&$-$ larg & .000&$-$ medi & .001&$-$ medi & .006\\
& best text vs All
& & .264& & .288&$+$ larg & .000& & .879&$+$ medi & .000& & .514\\
& best text vs best meta
& & .427& & .201& & .330& & .214&$+$ medi & .000& & .059\\
& Count vs All
&$+$ negl & .000& & .239&$+$ medi & .000& & .987&$+$ medi & .000& & .470\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& best text vs \#Add/Rem
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs Count
&$-$ larg & .000& & .022&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs Hist
&$-$ larg & .000& & .762& & .048&$-$ larg & .000& & .599& & .135\\
& best text vs All
&$-$ larg & .002&$-$ larg & .007&$+$ medi & .008& & .010& & .208&$-$ larg & .007\\
& best text vs best meta
&$-$ medi & .002& & .679& & .048& & .055&$+$ smal & .001& & .934\\
& Count vs All
&$+$ medi & .000& & .022&$+$ larg & .000& & .277&$+$ larg & .000& & .073\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& best text vs \#Add/Rem
&$-$ larg & .000& & .284&$-$ larg & .000& & .963&$-$ larg & .000& & .174\\
& best text vs Count
& & .130& & .347& & .014& & .016& & .090& & .580\\
& best text vs Hist
&$-$ larg & .000& & .011&$-$ larg & .000&$-$ larg & .006&$-$ larg & .000& & .021\\
& best text vs All
& & .081& & .347&$+$ larg & .001& & .024&$+$ larg & .000& & .030\\
& best text vs best meta
& & .081& & .347&$+$ larg & .001& & .024&$+$ larg & .000& & .030\\
& Count vs All
& & .026& & .355&$+$ smal & .005& & .243&$+$ medi & .000&$+$ larg & .001\\

\hline \hline 

\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{all}}}

& best text vs \#Add/Rem
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs Count
& & .095& & .024& & .850& & .120& & .091& & .201\\
& best text vs Hist
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs All
& & .675& & .503& & .018& & .338& & .140& & .598\\
& best text vs best meta
& & .936& & .688&$+$ larg & .001& & .071& & .127& & .131\\
& Count vs All
&$+$ smal & .000& & .050&$+$ smal & .002&$+$ medi & .001&$+$ medi & .000& & .012\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& best text vs \#Add/Rem
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs Count
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000&$-$ larg & .001&$-$ larg & .000& & .055\\
& best text vs Hist
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .008&$-$ larg & .001&$-$ larg & .000&$-$ larg & .000\\
& best text vs All
& & .048&$-$ larg & .007& & .421& & .421& & .252& & .524\\
& best text vs best meta
&$-$ larg & .008&$-$ medi & .007& & .277& & .804& & .252& & .389\\
& Count vs All
&$+$ larg & .000& & .599&$+$ larg & .008&$+$ larg & .005&$+$ larg & .008& & .107\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& best text vs \#Add/Rem
&$-$ larg & .000&$-$ larg & .000&$-$ larg & .009&$-$ larg & .000&$-$ larg & .000&$-$ larg & .000\\
& best text vs Count
& & .090& & .551&$+$ medi & .009& & .355& & .369& & .966\\
& best text vs Hist
&$-$ larg & .001&$-$ larg & .000&$-$ larg & .004&$-$ larg & .000&$-$ larg & .008&$-$ larg & .000\\
& best text vs All
& & .010& & .034&$+$ larg & .000& & .055&$+$ larg & .003& & .393\\
& best text vs best meta
& & .010& & .034&$+$ larg & .000& & .055&$+$ larg & .003& & .393\\
& Count vs All
&$+$ medi & .000&$+$ smal & .000&$+$ smal & .009& & .014&$+$ smal & .000& & .032\\
    \end{tabular}
% \end{sidewaystable}
\end{table}

==> tables/RQ3_mega_res.tex <==

% \begin{longtable}[!t]

%     \centering
    \begin{longtable}{ll|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c|p{.3cm}p{.3cm}p{.3cm}p{.3cm}p{.3cm}c}

    \caption{THIS TABLE WILL NOT BE IN THE PAPER, it is here just to see the full results for c}
        o\\
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{6}{c|}{commented}& \multicolumn{6}{c}{revised}& \multicolumn{6}{c}{Hotspot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        &auc&f1&gm&pre&rec&mod
        \\


\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}} 
& Baseline
&61& 9& 23& 38& 5&RF&68& 37& 53& 44& 32&RFs&65& 43& 56& 50& 37&RFs\\ \cline{2-20}
& Best text
&66& 34& 51& 39& 30&RFs&68& 41& 59& 41& 42&RFs&66& 48& 62& 42& 57\bestcell &RFs\\ 
& Best meta
&66& 33& 51& 37& 30&RFs&72\bestcell & 45\bestcell & 64\bestcell & 41& 52\bestcell &RFs&69\bestcell & 51\bestcell & 64\bestcell & 46& 57\bestcell &RFs\\ \cline{2-20}
&Count BoW +
&66& 31& 48& 40& 26&RFs&68& 38& 56& 40& 36&RFs&66& 44& 58& 46& 42&RFs\\ 
&Hist BoW +
&66& 35\bestcell & 54\bestcell & 36& 34\bestcell &RFs&70& 41& 59& 42& 41&RFs&67& 46& 60& 47& 45&RFs\\ 
&All BoW +
&67& 23& 38& 49& 15&RFs&71& 33& 47& 52\bestcell & 24&RFs&69\bestcell & 39& 52& 55& 30&RFs\\ 
&\#Add/Rem BoW +/-
&61& 9& 23& 37& 5&RF&68& 25& 40& 47& 17&RFs&65& 43& 57& 50& 38&RFs\\ 
&Count BoW +/-
&66& 30& 47& 41& 24&RFs&68& 36& 52& 42& 29&RFs&66& 45& 58& 48& 42&RFs\\ 
&Hist BoW +/-
&66& 34& 52& 36& 31&RFs&70& 39& 56& 43& 35&RFs&67& 44& 57& 50& 39&RFs\\ 
&All BoW +/-
&67& 20& 35& 50\bestcell & 13&RFs&71& 30& 45& 52\bestcell & 22&RFs&68& 39& 52& 59\bestcell & 29&RFs\\ 
&\#Add/Rem LLM +
&66& 34& 51& 39& 30&RFs&68& 40& 58& 40& 41&RFs&66& 47& 61& 47& 47&RFs\\ 
&Count LLM +
&68\bestcell & 19& 34& 42& 12&RFs&69& 28& 43& 46& 20&RFs&67& 34& 47& 55& 24&RFs\\ 
&Hist LLM +
&67& 32& 49& 41& 26&RFs&69& 28& 42& 52\bestcell & 19&RFs&67& 45& 58& 51& 40&RFs\\ 
&All LLM +
&68\bestcell & 20& 35& 45& 13&RFs&70& 30& 44& 52\bestcell & 21&RFs&68& 35& 48& 57& 25&RFs\\ 
&\#Add/Rem LLM +/-
&67& 33& 51& 38& 29&RFs&68& 41& 59& 40& 41&RFs&66& 47& 60& 46& 46&RFs\\ 
&Count LLM +/-
&68\bestcell & 19& 34& 46& 12&RFs&68& 32& 48& 44& 26&RFs&67& 33& 46& 54& 23&RFs\\ 
&Hist LLM +/-
&67& 31& 48& 40& 25&RFs&69& 28& 43& 51& 19&RFs&67& 46& 59& 52& 40&RFs\\ 
&All LLM +/-
&68\bestcell & 20& 35& 45& 13&RFs&69& 28& 43& 49& 20&RFs&68& 34& 47& 57& 24&RFs\\ 
\hline 
 

\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}} 
& Baseline
&79& 47& 70\bestcell & 38& 60\bestcell &RFs&68& 42& 60& 37& 51&RFs&72& 54& 66& 44& 69&RFs\\ \cline{2-20}
& Best text
&79& 48\bestcell & 70\bestcell & 42& 57&RFs&69& 46\bestcell & 64\bestcell & 39& 56&RFs&71& 54& 66& 44& 70\bestcell &RFs\\ 
& Best meta
&67& 30& 56& 24& 41&RFs&65& 41& 60& 33& 60\bestcell &RFs&71& 47& 60& 50& 45&RFs\\ \cline{2-20}
&Count BoW +
&79& 38& 56& 43& 35&RFs&69& 28& 44& 41& 21&RFs&73& 50& 62& 54& 46&RFs\\ 
&Hist BoW +
&78& 39& 56& 42& 34&RFs&75& 12& 25& 71& 7&RFs&78& 55& 67& 56& 54&RFs\\ 
&All BoW +
&80\bestcell & 31& 46& 56& 22&RFs&76\bestcell & 12& 25& 74& 7&RFs&80\bestcell & 43& 54& 70& 31&RFs\\ 
&\#Add/Rem BoW +/-
&79& 47& 70\bestcell & 39& 59&RFs&69& 43& 61& 39& 52&RFs&71& 54& 66& 44& 70\bestcell &RFs\\ 
&Count BoW +/-
&79& 36& 54& 42& 31&RFs&71& 35& 50& 48& 27&RFs&72& 51& 64& 50& 53&RFs\\ 
&Hist BoW +/-
&78& 40& 56& 41& 34&RFs&76\bestcell & 13& 26& 74& 7&RFs&78& 56& 67& 58& 53&RFs\\ 
&All BoW +/-
&79& 25& 41& 51& 17&RFs&76\bestcell & 14& 28& 67& 8&RFs&78& 30& 43& 75\bestcell & 19&RF\\ 
&\#Add/Rem LLM +
&79& 45& 63& 44& 44&RFs&68& 23& 38& 45& 15&RFs&72& 54& 66& 47& 65&RFs\\ 
&Count LLM +
&79& 35& 51& 48& 28&RFs&68& 26& 41& 46& 18&RFs&72& 48& 60& 53& 41&RFs\\ 
&Hist LLM +
&79& 43& 60& 45& 40&RFs&73& 8& 21& 69& 5&RFs&74& 55& 68& 51& 63&RFs\\ 
&All LLM +
&79& 33& 47& 61\bestcell & 22&RFs&73& 9& 22& 77& 5&RFs&75& 25& 39& 70& 15&RFs\\ 
&\#Add/Rem LLM +/-
&79& 43& 62& 42& 43&RFs&67& 24& 39& 43& 16&RFs&71& 54& 67& 47& 63&RFs\\ 
&Count LLM +/-
&79& 35& 51& 49& 28&RFs&67& 25& 40& 43& 17&RFs&72& 47& 59& 55& 41&RFs\\ 
&Hist LLM +/-
&78& 45& 60& 44& 40&RFs&72& 9& 21& 80\bestcell & 5&RFs&74& 57\bestcell & 69\bestcell & 49& 68&RFs\\ 
&All LLM +/-
&79& 31& 46& 54& 22&RFs&72& 10& 23& 76& 6&RFs&74& 31& 44& 66& 20&RFs\\ 
\hline 
 

\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}} 
& Baseline
&78& 34& 47& 57& 24&RFs&76& 47& 66& 43& 52&RFs&63& 48& 56& 53& 44&RFs\\ \cline{2-20}
& Best text
&78& 35& 48& 57& 25&RFs&78& 48\bestcell & 66& 44& 52&RFs&58& 50& 57& 48& 51&RF\\ 
& Best meta
&72& 54& 65& 47& 67\bestcell &RF&69& 43& 65& 35& 56&RFs&64& 55& 61& 52& 58&RFs\\ \cline{2-20}
&Count BoW +
&49& 36& 49& 57& 26&RFs&78& 47& 64& 47& 46&RFs&54& 47& 56& 60& 38&RFs\\ 
&Hist BoW +
&82\bestcell & 64& 73& 69\bestcell & 60&RFs&79& 46& 60& 57& 38&RFs&76& 67\bestcell & 71\bestcell & 63& 72\bestcell &RFs\\ 
&All BoW +
&74& 24& 37& 64& 15&RFs&79& 32& 45& 67& 20&RFs&64& 33& 45& 74& 22&RFs\\ 
&\#Add/Rem BoW +/-
&78& 34& 47& 57& 24&RFs&76& 46& 66& 42& 52&RFs&64& 48& 57& 53& 44&RFs\\ 
&Count BoW +/-
&48& 35& 48& 58& 25&RFs&78& 47& 64& 48& 47&RFs&54& 48& 57& 61& 39&RFs\\ 
&Hist BoW +/-
&82\bestcell & 65\bestcell & 73& 68& 61&RFs&79& 46& 60& 57& 39&RFs&77\bestcell & 67\bestcell & 71\bestcell & 64& 70&RFs\\ 
&All BoW +/-
&76& 24& 38& 66& 15&RFs&79& 31& 44& 68\bestcell & 20&RFs&64& 34& 46& 73& 22&RFs\\ 
&\#Add/Rem LLM +
&77& 33& 46& 57& 23&RFs&78& 47& 69\bestcell & 38& 62\bestcell &RFs&58& 49& 56& 47& 53&RFs\\ 
&Count LLM +
&49& 34& 47& 59& 24&RFs&78& 42& 57& 54& 35&RFs&55& 48& 57& 53& 43&RFs\\ 
&Hist LLM +
&81& 63& 74\bestcell & 63& 66&RFs&80\bestcell & 42& 56& 60& 33&RFs&77\bestcell & 65& 68& 64& 66&RFs\\ 
&All LLM +
&66& 18& 32& 66& 11&RFs&80\bestcell & 32& 45& 68\bestcell & 21&RFs&64& 29& 42& 78\bestcell & 18&RF\\ 
&\#Add/Rem LLM +/-
&78& 33& 46& 58& 22&RFs&78& 47& 69\bestcell & 38& 62\bestcell &RFs&58& 50& 56& 47& 53&RFs\\ 
&Count LLM +/-
&48& 37& 51& 54& 29&RFs&78& 43& 58& 54& 36&RFs&55& 49& 57& 54& 44&RFs\\ 
&Hist LLM +/-
&80& 63& 73& 63& 66&RFs&79& 43& 57& 58& 34&RFs&77\bestcell & 65& 70& 63& 67&RFs\\ 
&All LLM +/-
&63& 20& 34& 66& 12&RFs&80\bestcell & 25& 39& 65& 15&RFs&63& 34& 46& 76& 22&RF\\ 
\hline 
 

\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}} 
& Baseline
&74& 21& 36& 49\bestcell & 13&RFs&71& 27& 41& 58\bestcell & 18&RFs&68& 39& 53& 58\bestcell & 32&RFs\\ \cline{2-20}
& Best text
&76& 31& 54& 33& 33&RFs&71& 36& 51& 46& 28&RFs&67& 47& 59& 51& 40&RFs\\ 
& Best meta
&76& 33& 57& 30& 34&RFs&77& 44\bestcell & 64\bestcell & 44& 48\bestcell &RFs&71& 55\bestcell & 65\bestcell & 50& 59&RFs\\ \cline{2-20}
&Count BoW +
&81\bestcell & 38\bestcell & 59\bestcell & 41& 38\bestcell &RFs&78\bestcell & 44\bestcell & 60& 50& 39&RFs&75\bestcell & 53& 64& 55& 50&RFs\\ 
&Hist BoW +
&77& 34& 54& 39& 30&RFs&74& 41& 58& 44& 38&RFs&71& 48& 63& 53& 46&RFs\\ 
&All BoW +
&&&&&&&&&&&&&&&&&&\\ 
&\#Add/Rem BoW +/-
&73& 21& 37& 39& 15&RFs&71& 23& 38& 54& 15&RFs&68& 46& 59& 48& 43&RFs\\ 
&Count BoW +/-
&81\bestcell & 38\bestcell & 59\bestcell & 43& 37&RFs&78\bestcell & 43& 60& 49& 40&RFs&75\bestcell & 53& 64& 55& 51&RFs\\ 
&Hist BoW +/-
&76& 30& 50& 37& 26&RFs&73& 40& 58& 45& 38&RFs&70& 48& 62& 47& 50&RFs\\ 
&All BoW +/-
&&&&&&&&&&&&&&&&&&\\ 
&\#Add/Rem LLM +
&75& 34& 54& 36& 31&RFs&73& 36& 52& 46& 30&RFs&70& 53& 63& 47& 60&RFs\\ 
&Count LLM +
&81\bestcell & 34& 54& 35& 34&RFs&77& 40& 60& 42& 41&RFs&71& 53& 64& 51& 52&RFs\\ 
&Hist LLM +
&75& 25& 40& 36& 16&RFs&73& 39& 54& 40& 32&RFs&70& 49& 63& 48& 54&RFs\\ 
&All LLM +
&80& 34& 53& 36& 30&RFs&77& 34& 49& 46& 26&RFs&73& 50& 64& 51& 63\bestcell &RFs\\ 
&\#Add/Rem LLM +/-
&74& 26& 52& 30& 29&RFs&71& 30& 54& 44& 33&RFs&69& 47& 62& 42& 53&RFs\\ 
&Count LLM +/-
&80& 30& 48& 35& 25&RFs&77& 42& 60& 44& 42&RFs&72& 46& 59& 50& 42&RFs\\ 
&Hist LLM +/-
&76& 18& 33& 33& 11&RFs&72& 35& 53& 40& 32&RFs&70& 49& 63& 50& 54&RFs\\ 
&All LLM +/-
&79& 27& 45& 35& 21&RFs&76& 33& 49& 48& 25&RFs&72& 48& 59& 48& 41&RFs\\ 
\hline 
 

\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}} 
& Baseline
&72& 22& 38& 36& 15&RFs&70& 25& 41& 49& 17&RFs&66& 40& 54& 53& 32&RFs\\ \cline{2-20}
& Best text
&77& 26& 52& 31& 30&RFs&73& 37& 53& 48& 29&RFs&71& 49& 64& 49& 52&RFs\\ 
& Best meta
&79& 34& 58& 29& 37&RFs&77& 42& 62& 42& 45&RFs&74& 52& 65\bestcell & 47& 57&RFs\\ \cline{2-20}
&Count BoW +
&82\bestcell & 35\bestcell & 54& 44& 30&RFs&76& 40& 56& 49& 35&RFs&74& 50& 62& 52& 48&RFs\\ 
&Hist BoW +
&78& 30& 52& 38& 29&RFs&73& 36& 53& 47& 30&RFs&73& 51& 65\bestcell & 47& 55&RFs\\ 
&All BoW +
&&&&&&&&&&&&&&&&&&\\ 
&\#Add/Rem BoW +/-
&74& 22& 40& 37& 16&RFs&72& 26& 41& 50& 17&RFs&70& 47& 60& 48& 48&RFs\\ 
&Count BoW +/-
&82\bestcell & 35\bestcell & 53& 44& 29&RFs&75& 37& 53& 51\bestcell & 30&RFs&74& 50& 63& 54\bestcell & 48&RFs\\ 
&Hist BoW +/-
&75& 23& 40& 38& 16&RFs&72& 34& 50& 47& 27&RFs&70& 49& 63& 46& 54&RFs\\ 
&All BoW +/-
&&&&&&&&&&&&&&&&&&\\ 
&\#Add/Rem LLM +
&75& 31& 54& 32& 34&RFs&75& 43& 61& 48& 46\bestcell &RFs&70& 51& 59& 50& 59&RFs\\ 
&Count LLM +
&81& 35\bestcell & 59\bestcell & 33& 38\bestcell &RFs&78\bestcell & 37& 54& 44& 31&RFs&73& 52& 63& 46& 61&RFs\\ 
&Hist LLM +
&76& 23& 40& 39& 16&RFs&74& 37& 54& 42& 32&RFs&72& 51& 64& 43& 62&RFs\\ 
&All LLM +
&82\bestcell & 28& 46& 42& 21&RFs&78\bestcell & 40& 56& 46& 34&RFs&76\bestcell & 52& 64& 49& 63\bestcell &RFs\\ 
&\#Add/Rem LLM +/-
&75& 21& 35& 45\bestcell & 13&RFs&68& 39& 53& 48& 34&RFs&62& 51& 53& 54\bestcell & 47&RFs\\ 
&Count LLM +/-
&81& 34& 59\bestcell & 34& 38\bestcell &RFs&78\bestcell & 44\bestcell & 63\bestcell & 45& 43&RFs&74& 52& 65\bestcell & 50& 57&RFs\\ 
&Hist LLM +/-
&76& 25& 42& 34& 18&RFs&73& 39& 57& 40& 37&RFs&70& 50& 64& 44& 60&RFs\\ 
&All LLM +/-
&81& 27& 44& 41& 20&RFs&77& 39& 55& 44& 33&RFs&74& 54\bestcell & 64& 47& 59&RFs\\ 
\hline 
 
    \end{longtable}
    % \caption{Description of the revision activity on the studied project}
    % \label{tab:rev_activity}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{lll|ccccc|ccccc}
%         &Embed&Mod
%         &\multicolumn{5}{c|}{commented}& \multicolumn{5}{c}{revised}
%         \\
%         &&
%         &AUC&F1&GM&Pre&Rec
%         &AUC&F1&GM&Pre&Rec\\

%     \hline
%     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}}
%     & Baseline &
%     &&&&
%     &&&&\\
%     & Best text &
%     &&&&
%     &&&&\\
%     & Best soft &
%     &&&&
%     &&&&\\
%     & Best combi &
%     &&&&
%     &&&&\\

%     \hline
%     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}}
%     & Baseline &
%     &&&&
%     &&&&\\
%     & Best text &
%     &&&&
%     &&&&\\
%     & Best soft &
%     &&&&
%     &&&&\\
%     & Best combi &
%     &&&&
%     &&&&\\

    
%     \hline
%     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}}
%     & Baseline &
%     &&&&
%     &&&&\\
%     & Best text &
%     &&&&
%     &&&&\\
%     & Best soft &
%     &&&&
%     &&&&\\
%     & Best combi &
%     &&&&
%     &&&&\\

    
%     \hline
%     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}}
%     & Baseline &
%     &&&&
%     &&&&\\
%     & Best text &
%     &&&&
%     &&&&\\
%     & Best soft &
%     &&&&
%     &&&&\\
%     & Best combi &
%     &&&&
%     &&&&\\
    
%     \hline
%     \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}}
%     & Baseline &
%     &&&&
%     &&&&\\
%     & Best text &
%     &&&&
%     &&&&\\
%     & Best soft &
%     &&&&
%     &&&&\\
%     & Best combi &
%     &&&&
%     &&&&\\
    
%     \end{tabular}
%     \caption{Description of the revision activity on the studied project}
%     \label{tab:rev_activity}
% \end{longtable}

==> tables/RQ3_res.tex <==


\begin{table}[t]
    \centering
    \small
    \caption{Results of combining the text embeddings with software meta-features embeddings on the code review activity prediction task. The results are returned for the best model ("mod") for each setting of text embedding. The results of the median F1-score are reported. Blue cells indicate the maximum values for each metric by dataset and by label.}
    \label{tab:RQ3_res}
    
    \begin{tabularx}{\textwidth}{Xl|XXXXXc|XXXXXc|XXXXXc}
        \hline
        &\multicolumn{1}{c|}{\textbf{Text}}
        &\multicolumn{6}{c|}{\textbf{Commented}}& \multicolumn{6}{c|}{\textbf{Revised}}& \multicolumn{6}{c}{\textbf{Hot-spot}}
        \\
        & \multicolumn{1}{c|}{\textbf{Embed}}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        &\textbf{auc}&\textbf{f1}&\textbf{gm}&\textbf{pre}&\textbf{rec}&\textbf{mod}
        \\




% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}} 
% & Baseline
% &64& 37& 60& 31\samecell & 48&RFs&68& 43& 63& 35\samecell & 53&RFs&65& 48& 62\samecell & 42\samecell & 57&RFs\\ \cline{2-20}
% & Best text
% &67& 39\samecell & 63\bestcell & 28\samecell & 66\samecell &RFs&69& 43& 64& 32\samecell & 66\samecell &RFs&66& 49& 62\samecell & 42\samecell & 58\samecell &RFs\\ 
% & Best feat
% &66& 38& 61& 29\samecell & 56&RF&73\bestcell & 45\bestcell & 66\bestcell & 36\bestcell & 62\samecell &RF&70\bestcell & 51\bestcell & 63\samecell & 40\samecell & 73\samecell &RF\\ \cline{2-20}
% & Combi auc
% &68\bestcell & 40\bestcell & 62\samecell & 29\samecell & 60\samecell &RFs&71& 43& 64\samecell & 36\samecell & 54\samecell &RF&68& 51& 63\bestcell & 40\samecell & 68\samecell &RFs\\  
% &&\multicolumn{6}{|c}{LLM + $\&$ Count}&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% & Combi f1
% &68\bestcell & 40\bestcell & 62\samecell & 29\samecell & 60\samecell &RFs&71\samecell & 44& 65& 34\samecell & 61\samecell &RFs&68\samecell & 51\samecell & 63\bestcell & 40\samecell & 68\samecell &RFs\\  
% &&\multicolumn{6}{|c}{LLM + $\&$ Count}&\multicolumn{6}{|c}{WC +/- $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% \hline 
 

% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}} 
% & Baseline
% &79& 47& 70& 40\bestcell & 60\samecell &RFs&68& 48& 66& 35& 77\bestcell &RFs&72& 55& 65& 42& 84\samecell &RF\\ \cline{2-20}
% & Best text
% &79& 48\samecell & 72& 36\samecell & 69\samecell &RFs&69& 48& 66& 37& 69&RFs&72& 55& 66& 43& 74&RFs\\ 
% & Best feat
% &75& 41& 66& 32& 54\samecell &RF&73\samecell & 49& 67& 37& 73&RFs&76& 57& 67& 43& 84\samecell &RFs\\ \cline{2-20}
% & Combi auc
% &80\bestcell & 47& 71& 37& 63\samecell &RF&74\bestcell & 51\bestcell & 69\bestcell & 40\samecell & 74&RFs&78\bestcell & 59\samecell & 71\samecell & 49\samecell & 76\samecell &RF\\  
% &&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% & Combi f1
% &79& 49\bestcell & 73\samecell & 38\samecell & 67\samecell &RFs&74\bestcell & 51\bestcell & 69\bestcell & 40\samecell & 74&RFs&78\samecell & 60\bestcell & 70\samecell & 46\samecell & 85\bestcell &RFs\\  
% &&\multicolumn{6}{|c}{LLM + $\&$ Count}&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ Hist}\\ 
% \hline 
 

% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}} 
% & Baseline
% &79\bestcell & 65\bestcell & 75\bestcell & 62\bestcell & 69&RFs&76& 47& 64& 45\samecell & 47&RFs&63\samecell & 61\samecell & 50& 46\samecell & 92&RFs\\ \cline{2-20}
% & Best text
% &78& 65\samecell & 75\samecell & 59\samecell & 73&RFs&78& 48& 66\samecell & 44& 52\samecell &RFs&64\bestcell & 61\samecell & 51& 46\samecell & 92&RFs\\ 
% & Best feat
% &56& 50& 55& 36& 82&RFs&77& 48& 70\bestcell & 37& 66\bestcell &RFs&57& 58& 45& 44\samecell & 89&RF\\ \cline{2-20}
% & Combi auc
% &78& 65\samecell & 75\samecell & 59\samecell & 74&RFs&79\bestcell & 49\samecell & 68\samecell & 45\samecell & 55\samecell &RFs&64\samecell & 61\bestcell & 51& 46\samecell & 91&RFs\\  
% &&\multicolumn{6}{|c}{WC +/- $\&$ Add/Rem}&\multicolumn{6}{|c}{LLM + $\&$ All}&\multicolumn{6}{|c}{WC +/- $\&$ Add/Rem}\\ 
% & Combi f1
% &78& 65\samecell & 75\samecell & 59\samecell & 74&RFs&78& 50\bestcell & 68\samecell & 46\bestcell & 54\samecell &RFs&64\samecell & 61\bestcell & 51& 46\samecell & 91&RFs\\  
% &&\multicolumn{6}{|c}{WC +/- $\&$ Add/Rem}&\multicolumn{6}{|c}{WC +/- $\&$ Hist}&\multicolumn{6}{|c}{WC +/- $\&$ Add/Rem}\\ 
% \hline 
 

% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}} 
% & Baseline
% &&&&&&&&&&&&&&&&&&\\ \cline{2-20}
% & Best text
% &76\samecell & 36& 66& 30\samecell & 51&RFs&72& 45& 66& 38& 57&RFs&69\samecell & 53\samecell & 63\samecell & 43\samecell & 68&RFs\\ 
% & Best feat
% &59& 27& 54& 15& 78\bestcell &RF&59& 37& 41& 23& 96\bestcell &RF&61& 51& 34& 35& 99\bestcell &RF\\ \cline{2-20}
% & Combi auc
% &80\bestcell & 41\samecell & 68\samecell & 33\samecell & 58\samecell &RFs&78\bestcell & 51\samecell & 70& 41\samecell & 67&RFs&73\bestcell & 58\bestcell & 67\bestcell & 49\bestcell & 71&RFs\\  
% &&\multicolumn{6}{|c}{LLM + $\&$ All}&\multicolumn{6}{|c}{WC +/- $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% & Combi f1
% &80\samecell & 44\bestcell & 68\samecell & 36\samecell & 53\samecell &RFs&78\samecell & 52\bestcell & 71\bestcell & 41\bestcell & 66&RFs&73\bestcell & 58\bestcell & 67\bestcell & 49\bestcell & 71&RFs\\  
% &&\multicolumn{6}{|c}{WC +/- $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% \hline 
 

% \hline 
% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}} 
% & Baseline
% &&&&&&&&&&&&&&&&&&\\ \cline{2-20}
% & Best text
% &77& 34& 64& 26\samecell & 48\samecell &RFs&73& 42& 67& 34& 65&RFs&71& 52& 63& 41\samecell & 72\samecell &RFs\\ 
% & Best feat
% &60& 22& 57& 13& 71\bestcell &RFs&62& 36& 59& 24& 74\bestcell &RFs&66& 50& 63& 38& 77\samecell &RFs\\ \cline{2-20}
% & Combi auc
% &82\bestcell & 43\bestcell & 67& 37\bestcell & 50&RFs&80\bestcell & 48\samecell & 71\bestcell & 41\samecell & 62&RFs&79\bestcell & 56& 71\bestcell & 46\samecell & 74&RF\\  
% &&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{WC + $\&$ All}\\ 
% & Combi f1
% &82\bestcell & 43\bestcell & 67& 37\bestcell & 50&RFs&76\samecell & 51\bestcell & 68\samecell & 42\bestcell & 64\samecell &RFs&67& 60\bestcell & 58& 47\bestcell & 79\samecell &RF\\  
% &&\multicolumn{6}{|c}{WC + $\&$ All}&\multicolumn{6}{|c}{LLM +/- $\&$ All}&\multicolumn{6}{|c}{LLM +/- $\&$ All}\\ 
% \hline 

\hline 
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Base}}} 
& Baseline
&61& 9& 23& 38& 5&RF&68& 37& 53& 44 \bestcell& 32&RFs&65& 43& 56& 50 \bestcell& 37&RFs\\ \cline{2-20}
& Best text
&66 \bestcell& 34& 51& 39 \bestcell& 30&RFs&68& 41& 59& 41& 42&RFs&66& 48& 62& 42& 57\bestcell &RFs\\ 
& Best feat
&66 \bestcell& 33& 51& 37& 30&RFs&72\bestcell & 45\bestcell & 64\bestcell & 41& 52\bestcell &RFs&69\bestcell & 51\bestcell & 64\bestcell & 46& 57\bestcell &RFs\\ \cline{2-20}
% &Default combi&68\bestcell & 20& 35& 45& 13&RFs&69& 28& 43& 49& 20&RFs&68& 34& 47& 57& 24&RFs\\ 
& Best combi
&66 \bestcell& 35\bestcell & 54\bestcell & 36& 34\bestcell &RFs&70& 41& 59& 42& 41&RFs&66& 47& 61& 47& 47&RFs\\  
&&\multicolumn{6}{|c}{BoW + $\&$ Hist}&\multicolumn{6}{|c}{BoW + $\&$ Hist}&\multicolumn{6}{|c}{LLM + $\&$ Add/Rem}\\ 
  
\hline 
\hline 

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Ironic}}} 
& Baseline
&79 \bestcell& 47& 70\bestcell & 38& 60\bestcell &RFs&68 & 42& 60& 37& 51&RFs&72& 54& 66& 44& 69&RFs\\ \cline{2-20}
& Best text
&79 \bestcell& 48\bestcell & 70\bestcell & 42& 57&RFs&69 \bestcell& 46\bestcell & 64\bestcell & 39 \bestcell& 56&RFs&71& 54& 66& 44& 70\bestcell &RFs\\ 
& Best feat
&67& 30& 56& 24& 41&RFs&65& 41& 60& 33& 60\bestcell &RFs&71& 47& 60& 50 \bestcell& 45&RFs\\ \cline{2-20}
% &Default combi&79& 31& 46& 54& 22&RFs&72& 10& 23& 76& 6&RFs&74& 31& 44& 66& 20&RFs\\ 
& Best combi
&79 \bestcell& 47& 70\bestcell & 39 \bestcell& 59&RFs&69\bestcell& 43& 61& 39 \bestcell& 52&RFs&74 \bestcell& 57\bestcell & 69\bestcell & 49& 68&RFs\\  
&&\multicolumn{6}{|c}{BoW +/- $\&$ Add/Rem}&\multicolumn{6}{|c}{BoW +/- $\&$ Add/Rem}&\multicolumn{6}{|c}{LLM +/- $\&$ Hist}\\  
\hline 
\hline 

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Nova}}} 
& Baseline
&78& 34& 47& 57& 24&RFs&76& 47& 66\bestcell& 43& 52&RFs&63& 48& 56& 53& 44&RFs\\ \cline{2-20}
& Best text
&78& 35& 48& 57& 25&RFs&78 \bestcell& 48\bestcell & 66 \bestcell& 44& 52&RFs&58& 50& 57& 48& 51&RF\\ 
& Best feat
&72& 54& 65& 47& 67\bestcell &RF&69& 43& 65& 35& 56 \bestcell&RFs&64& 55& 61& 52& 58&RFs\\ \cline{2-20}
% &Default combi&78& 33& 46& 58& 22&RFs&78& 47& 69\bestcell & 38& 62\bestcell &RFs&58& 50& 56& 47& 53&RFs\\  
& Best combi
&82\bestcell & 65\bestcell & 73 \bestcell& 68 \bestcell& 61&RFs&78 \bestcell& 47& 64& 48 \bestcell& 47&RFs&76 \bestcell& 67\bestcell & 71\bestcell & 63 \bestcell& 72\bestcell &RFs\\  
&&\multicolumn{6}{|c}{BoW +/- $\&$ Hist}&\multicolumn{6}{|c}{BoW +/- $\&$ Count}&\multicolumn{6}{|c}{BoW + $\&$ Hist}\\
\hline 
\hline 

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed1}}} 
& Baseline
&74& 21& 36& 49\bestcell & 13&RFs&71& 27& 41& 58\bestcell & 18&RFs&68& 39& 53& 58\bestcell & 32&RFs\\ \cline{2-20}
& Best text
&76& 31& 54& 33& 33&RFs&71& 36& 51& 46& 28&RFs&67& 47& 59& 51& 40&RFs\\ 
& Best feat
&76& 33& 57& 30& 34&RFs&77& 44\bestcell & 64\bestcell & 44& 48\bestcell &RFs&71& 55\bestcell & 65\bestcell & 50& 59\bestcell&RFs\\ \cline{2-20}
% &Default combi&74& 26& 52& 30& 29&RFs&71& 30& 54& 44& 33&RFs&69& 47& 62& 42& 53&RFs\\ 
& Best combi
&81\bestcell & 38\bestcell & 59\bestcell & 41& 38\bestcell &RFs&78\bestcell & 44\bestcell & 60& 50& 39&RFs&75\bestcell & 53& 64& 55& 50&RFs\\  
&&\multicolumn{6}{|c}{BoW + $\&$ Count}&\multicolumn{6}{|c}{BoW + $\&$ Count}&\multicolumn{6}{|c}{BoW + $\&$ Count}\\  
\hline 
\hline 

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Closed2}}} 
& Baseline
&72& 22& 38& 36& 15&RFs&70& 25& 41& 49 \bestcell& 17&RFs&66& 40& 54& 53\bestcell& 32&RFs\\ \cline{2-20}
& Best text
&77& 26& 52& 31& 30&RFs&73& 37& 53& 48& 29&RFs&71& 49& 64& 49& 52&RFs\\ 
& Best feat
&79& 34& 58 \bestcell& 29& 37 \bestcell&RFs&77& 42& 62& 42& 45\bestcell&RFs&74 \bestcell& 52& 65\bestcell & 47& 57&RFs\\ \cline{2-20}
% &Default combi&75& 21& 35& 45\bestcell & 13&RFs&68& 39& 53& 48& 34&RFs&62& 51& 53& 54\bestcell & 47&RFs\\ 
& Best combi
&82\bestcell & 35\bestcell & 54& 44 \bestcell& 30&RFs&78\bestcell & 44\bestcell & 63\bestcell & 45& 43&RFs&74 \bestcell& 54\bestcell & 64& 47& 59\bestcell&RFs\\  
&&\multicolumn{6}{|c}{BoW + $\&$ Count}&\multicolumn{6}{|c}{LLM +/- $\&$ Count}&\multicolumn{6}{|c}{LLM +/- $\&$ All}\\ 
\hline 
 



    \end{tabularx}
    
\end{table}


==> tables/RQ3_stats.tex <==
\begin{table}[t]
% \begin{sidewaystable}
    \centering
\small
    \caption{Stat RQ3.}
    \label{RQ1:res}
        \begin{tabular}{ll|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}|
    p{.9cm}p{.3cm}p{.9cm}p{.3cm}}
        &\multicolumn{1}{c|}{Text}
        &\multicolumn{4}{c|}{commented}& \multicolumn{4}{c}{revised}& \multicolumn{4}{c}{hot-spot}
        \\
        & \multicolumn{1}{c|}{Embed}
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        &auc&p-val&f1&p-val
        \\

\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{all}}}

& baseline vs best text
&$+$ negl & .003& & .023&$+$ smal & .003&$+$ medi & .000& & .116&$+$ medi & .003\\
& baseline vs best meta
& & .806&$+$ medi & .000& & .035&$+$ larg & .000&$+$ medi & .000&$+$ larg & .001\\
& baseline vs default
& & .232& & .806&$+$ medi & .000& & .154&$+$ smal & .002& & .207\\
& baseline vs best combi
&$+$ larg & .000&$+$ larg & .000&$+$ larg & .000&$+$ larg & .000&$+$ larg & .000&$+$ larg & .000\\
& best meta vs best combi
&$+$ larg & .000&$+$ medi & .000& & .041& & .427& & .136& & .177\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& baseline vs best text
& & .135& & .041&$+$ smal & .003&$+$ medi & .000& & .041&$+$ medi & .002\\
& baseline vs best meta
&$-$ medi & .008&$+$ smal & .008& & .064& & .599& & .055& & .229\\
& baseline vs default
& & .599& & .083&$+$ larg & .000&$-$ larg & .000&$+$ smal & .008&$-$ larg & .000\\
& baseline vs best combi
&$+$ smal & .002&$+$ larg & .002&$+$ larg & .000& & .252&$+$ larg & .000&$+$ larg & .000\\
& best meta vs best combi
&$+$ medi & .008&$+$ larg & .000&$+$ larg & .008& & .421& & .041& & .015\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& baseline vs best text
& & .035& & .284& & .132& & .027& & .963& & .089\\
& baseline vs best meta
&$+$ larg & .004&$+$ larg & .000&$+$ larg & .000&$+$ larg & .000&$+$ larg & .001&$+$ larg & .000\\
& baseline vs default
& & .030& & .522& & .021& & .245& & .083& & .312\\
& baseline vs best combi
&$+$ larg & .000&$+$ larg & .001&$+$ larg & .000&$+$ larg & .000&$+$ larg & .001&$+$ larg & .004\\
& best meta vs best combi
&$+$ larg & .000& & .013& & .865& & .640& & .708& & .838\\


\hline \hline 
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{all}}}

& baseline vs best text
& & .562& & .822& & .053&$+$ smal & .010& & .322& & .067\\
& baseline vs best meta
& & .394& & .974&$+$ larg & .000&$+$ medi & .000& & .042&$+$ smal & .004\\
& baseline vs default
&$+$ medi & .000& & .781&$+$ smal & .004&$+$ medi & .001&$+$ smal & .003&$+$ smal & .003\\
& baseline vs best combi
&$+$ larg & .000&$+$ medi & .000&$+$ medi & .000&$+$ medi & .000&$+$ medi & .001&$+$ larg & .000\\
& best meta vs best combi
&$+$ medi & .004&$+$ medi & .000& & .604& & .033& & .071&$+$ smal & .002\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{open}}}

& baseline vs best text
&$-$ smal & .004& & .330& & .048&$+$ medi & .001& & .121& & .041\\
& baseline vs best meta
&$-$ larg & .008&$-$ medi & .008& & .095&$+$ medi & .004& & .890& & .389\\
& baseline vs default
&$+$ smal & .008& & .048& & .524& & .095&$+$ medi & .000& & .421\\
& baseline vs best combi
&$+$ medi & .002& & .015&$+$ larg & .000&$+$ medi & .003&$+$ medi & .000& & .010\\
& best meta vs best combi
&$+$ larg & .003&$+$ larg & .002& & .454& & .890&$+$ larg & .008& & .083\\
\hline
 \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{closed}}}

& baseline vs best text
& & .284& & .611& & .368& & .452& & .782& & .306\\
& baseline vs best meta
&$+$ larg & .000&$+$ medi & .004&$+$ larg & .000& & .012&$+$ medi & .006&$+$ medi & .004\\
& baseline vs default
& & .014& & .097&$+$ medi & .009&$+$ medi & .002& & .123&$+$ larg & .004\\
& baseline vs best combi
&$+$ larg & .000&$+$ larg & .000&$+$ medi & .009&$+$ medi & .002& & .083&$+$ larg & .001\\
& best meta vs best combi
& & .412&$+$ medi & .000& & .000&$+$ smal & .006& & .393&$+$ smal & .004\\
    \end{tabular}
% \end{sidewaystable}
\end{table}
